AutoLR: Layer-wise Pruning and Auto-tuning of Learning Rates in Fine-tuning of Deep Networks

Existing fine-tuning methods use a single learning rate over all layers. In this paper, first, we discuss that trends of layer-wise weight variations by fine-tuning using a single learning rate do not match the well-known notion that lower-level layers extract general features and higher-level layers extract specific features. Based on our discussion, we propose an algorithm that improves fine-tuning performance and reduces network complexity through layer-wise pruning and auto-tuning of layer-wise learning rates. The proposed algorithm has verified the effectiveness by achieving state-of-the-art performance on the image retrieval benchmark datasets (CUB-200, Cars-196, Stanford online product, and Inshop). Code is available at https://github.com/youngminPIL/AutoLR.

==> input_fig/Architure.tex <==
\begin{figure*}[t]
\centering
{\includegraphics[width=13.0cm]{fig/architecture_process4.pdf}}
%     \vspace{-0.5cm}
\caption{Architecture and Process}
    \label{fig:Architure}
\end{figure*}

==> input_fig/full_cam.tex <==
\begin{figure}[t]
\centering
{\includegraphics[width=6cm]{fig/full_cam.pdf}}
    \hfill    
    \caption{CAM for all layers}
    \label{fig:full_cam}
    \vspace{-0.4cm}
\end{figure}

==> input_tables/fine_grained_AutoLR.tex <==
\begin{table}[t]
\centering
\caption{The classification accuracy for applying Layer-wise pruning and AutoLR to Fine-grained classification task} %(ResNet-50 used, $\dagger$H means head of hydra structure)}
\label{table:fine-grained_autolr}
\vspace{+1mm}
% \footnotesize{
% \resizebox{1\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
ResNet-50       & \multicolumn{1}{c|}{CUB-200} & \multicolumn{1}{c|}{Cars-196} & \multicolumn{1}{c}{Aircraft}\\ \midrule
None pruned & 78.36     & 83.93  & 77.05       \\ 
Pruned 16 & 78.53   &84.70     & 77.67      \\ 
Pruned 15,16 & 78.79      &85.55    & 77.65  \\ \midrule
Pruned 15,16 + \textbf{AutoLR}	  &\textbf{79.98}    &\textbf{87.90}     & \textbf{81.94}	   \\ \bottomrule
\end{tabular}
% }
 \vspace{-0.2cm}
\end{table}

==> input_tables/finegrained_sota.tex <==
\begin{table}[t]
\caption{The comparison results (Top-1 Accuracy) with existing methods on fine-grained classification dataset, $\dagger$ indicates the case using additional network module.
}
\resizebox{0.5\textwidth}{!}{
\label{table:fine-grained_sota}
\centering
\begin{tabular}{lccccc}
\toprule
Method 	&Network	& ST-Car & Air 	 & CUB-C	   \\ \midrule
RA-CNN~\cite{ref:RA_CNN}&VGG-19$^\dagger$  &92.5 &88.2  &85.3 \\
MA-CNN~\cite{ref:MA_CNN}&VGG-19$^\dagger$  & 92.8 & 89.9  &86.5 \\ 
DT-RAM~\cite{ref:dt-ram}&ResNet-50$^\dagger$    &93.1 &- &86.0\\
DFL-CNN\cite{ref:dfl_cnn}&ResNet-50$^\dagger$   & 93.1 & \underline{91.7} &87.4\\
iSort-Cov~\cite{ref:iSORT_cov} &ResNet-101 &93.3 &91.4 & \textbf{88.7}\\
NTS-Net~\cite{ref:nts-net} &ResNet-50$^\dagger$ & \textbf{93.9} &91.4 & \underline{87.5} \\\midrule
Spot-tune\cite{ref:spot-tune}  &ResNet-50$^\dagger$	
& 92.4%0    
& -   &84.0%3   
\\ 
\textbf{Pruning only} & ResNet-50  &93.0%1
&89.5%2.  
& 84.6%8
\\ 
\textbf{Proposed}& ResNet-50   & \underline{93.8}%3 
&\textbf{91.8}%8}	 
&84.9%2	
\\\bottomrule
% Block3 + FC & 75.70			 & 90.26     &\textbf{96.76}&\textbf{97.92} \\
% Block4 + FC & 74.85 		& 90.14 		&96.32 				&97.71\\
% Block5 + FC & 73.39 		& 89.28 		&95.28 				&97.18\\ 
\end{tabular} }
\end{table}
% \begin{tablenotes}
%     	  		\footnotesize
%     	  	 	\item Note) Baseline is a fine-tuning using a fixed learning rate with dropping.
%     		\end{tablenotes}





% \begin{table}[t]
% \caption{The comparison results on fine-grained visual recognition dataset}
% \label{table:fine-grained}
% \centering
% \begin{tabular}{ccccc}
% \toprule
% model 		& ST-Car		& Aircraft 	 &CUB-FGVR		   \\ \midrule
% RA-CNN\cite{ref:RA_CNN}  &92.5 &88.2 & 85.3 \\
% MA-CNN\cite{ref:MA_CNN}   		& 92.8          & 89.9  & 86.5 \\ 
% DT-RAM    &93.1 &- &86.0\\
% NTS-Net & 93.9 &91.4& \textbf{87.5}\\
% DFL-CNN & 93.1 & 91.7 &87.4\\\midrule
% Spot-tune\cite{ref:spot-tune}   		& 92.40          & -     & 84.03\\ 
% Our     & \textbf{93.98} 	&\textbf{91.81}	 & 84.81   		 \\\bottomrule
% % Block3 + FC & 75.70			 & 90.26     &\textbf{96.76}&\textbf{97.92} \\
% % Block4 + FC & 74.85 		& 90.14 		&96.32 				&97.71\\
% % Block5 + FC & 73.39 		& 89.28 		&95.28 				&97.18\\ 
% \end{tabular}	
% \end{table}


==> input_tables/finegrained_spot.tex <==
\begin{table}[t]
\caption{The comparison results on fine-grained classification dataset (Top-1 Accuracy)}
\label{table:fine-grained_spot}
\centering
\begin{tabular}{ccccc}
\toprule
Model 		& Stanford Cars	&CUB-Class		& Aircraft 	 	   \\ \midrule
Spot-tune~\cite{ref:spot-tune}   & 92.40 & 84.03 & - \\
 \midrule
 Baseline & 92.81 	    &84.58          & 90.52  		 \\
Proposed     & \textbf{93.83}& \textbf{84.92}& \textbf{91.78}  		 \\
\bottomrule


% Block3 + FC & 75.70			 & 90.26     &\textbf{96.76}&\textbf{97.92} \\
% Block4 + FC & 74.85 		& 90.14 		&96.32 				&97.71\\
% Block5 + FC & 73.39 		& 89.28 		&95.28 				&97.18\\ 
\end{tabular}	
\end{table}


==> input_tables/pre_robustness.tex <==
\begin{table}[t]
\caption{The variance value of loss caused by applying random perturbation to each layer.\ro{100개씩 뽑는 것으로 새로 실험을 돌려서 채우는 중입니다. }}
\label{table:robustness}
\centering
\begin{tabular}{ccccc}
\toprule
target layers  &dimension  		& 20\% 		& 50\% 			   \\ \midrule
%0 (1.0)     & -		& 50.7914xe-8          & -          & -   \\ 
1 (1.0)     & 4,096		& 6.0375xe-8          & 38.4738xe-8     \\ 
2 (1.1)    & 16,384		& 0.7719xe-8          & 21.0402             \\ 
3 (1.2)   & 16,384	       & 1.2262xe-8          & 16.4596             \\
4 (2.0)    & 32,768		& 2.2472xe-8          & 14.0756xe-8  \\ 
5 (2.1)    & 65,536		& 0.6207xe-8          & 9.0588             \\ 
6 (2.2)    & -		& 0.9168xe-8          & 7.5925             \\ 
7 (2.3)    & -		& 0.9072xe-8          & -             \\ 
8 (3.0)     & -		& 3.3990xe-8          & 20.6008xe-8     \\ 
9 (3.1)     & -		& 0.7664xe-8          & 12.5131            \\ 
10 (3.2)    & - 		& 0.5159xe-8		& 9.3011		 \\
11 (3.3)    & - 		& 0.5059xe-8		& -		 \\
12 (3.4)    & - 		& 1.1137xe-8		& -		 \\
13 (3.5)    & - 		& 1.9481xe-8		& -		 \\
14 (4.0). & 524,288 		& 3.6990xe-8		& 21.3148xe-8\\
15 (4.1). & 1,048,576		& 1.9087xe-8		& 17.8357xe-8		 \\
16 (4.2) & 1,048,576        & 4.3756xe-8 	&- 			 \\\bottomrule
% Block3 + FC & 75.70			 & 90.26 &\textbf{96.76}&\textbf{97.92} \\
% Block4 + FC & 74.85 		& 90.14 		&96.32 				&97.71\\
% Block5 + FC & 73.39 		& 89.28 		&95.28 				&97.18\\ 
\end{tabular}	

\resizebox{0.5\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
samples &1(1.0)  & 10(3.2)	& 16(4.2)	   \\ \midrule
1     & 0.09789787917114544	& 0.09706286396024695  & 0.09976277973894371 \\ 
20    & 0.09726027909727518	& 0.09735262946848125  & 0.09791156635702326 \\ 
100   & 0.09730765984507195 & 0.09743554092780587  & 0.09795251116667962\\
500   & 0.09730179141529882	& 0.09742226564709713  & 0.09783841478458094 \\ 
1000  & 0.09723819788444982	& 0.09742133040490583  & 0.09788182047669317 \\ 
2000  & 0.09724988073751063 & 0.09742265217460461  & 0.09788768544828852 \\ 
3000  & 0.09728228342806017	& 0.0974208301914188  & 0.09788504567921964  \\
4000  & 0.09727309027566315	& 0.0974208301914188  & -             \\


\bottomrule

\end{tabular}	
}
\end{table}


==> input_tables/results_of_retrieval.tex <==
\begin{table*}[t]
\centering
\caption{Results of CUB and AIR}
\label{tabular:series}
\begin{tabular}{cccccc}
\toprule
Method     	& SOP	& CUB  & inshop  & BBBB  \\ \midrule
baseline	   & 77.17 	& 79.09  & 63.26 & 80.83   \\
tail-cut	    	   & 81.71 	& 83.02  & 66.09 & 81.96   \\
tail-cut + tailored	     	& 79.58    & 82.57   & \textbf{66.57}  & \textbf{82.41} \\
tail-cut + tailored$\dagger$	 &\textbf{80.34} &\textbf{84.49} & 66.39& 82.32  \\ \bottomrule
\end{tabular}

\label{tabular:series}
\begin{tabular}{ccccc}
\toprule
Method     	& SOP	& CUB  & inshop    \\ \midrule
baseline	   & 79.70 	& 79.09  & 63.26    \\
\bottomrule
\end{tabular}

\caption{Results our scheme on Stanford online products dataset}
\begin{tabular}{cccccc}
\toprule
Method     	& R@1	& R@10  & R@$10^2$  & R@$10^3$  \\ \midrule
baseline	   & 80.02 	& 91.21  & 96.20 & 98.64   \\
tail-cut	    	   & 81.71 	& 91.90  & 96.23 & 98.62   \\
tail-cut + tailored	     	& 83.70    & 92.80   & 96.64  & 98.66 \\
tail-cut + tailored$\dagger$	 &\textbf{84.14} &\textbf{93.36} & \textbf{96.88}& \textbf{98.80}  \\ \bottomrule
\end{tabular}

\caption{Results our scheme on CUB200 dataset}
\begin{tabular}{cccccc}
\toprule
Method     	& R@1	& R@2  & R@4  & R@8  \\ \midrule
baseline	   & 52.55 	& 65.60  & 76.65 & 85.40   \\
tail-cut	    	   & 66.22 	& 77.62  & 85.43 & 91.64   \\
tail-cut + tailored		& \textbf{69.45}    & \textbf{80.27}   & \textbf{87.47}  & \textbf{92.84} \\
tail-cut + tailored	 &69.35 &79.88 & 87.36& 92.66  \\ \bottomrule
\end{tabular}


\caption{Results our scheme on Inshop retrieval dataset}
\begin{tabular}{cccccc}
\toprule
Method     	& R@1	& R@10  & R@20  & R@30  \\ \midrule
baseline	   & 90.00 	& 97.47  & 98.30 & 98.61   \\
tail-cut	   & 91.28 	& 97.97  & 98.65 & 98.86   \\
tail-cut + tailored		& 69.45    & 80.27   & 87.47  & 92.84 \\
tail-cut + tailored	 &\textbf{84.14} &\textbf{93.36} & \textbf{96.88}& \textbf{98.80}  \\ \bottomrule
\end{tabular}


\caption{Results tail-cut Stanford online products dataset}
\begin{tabular}{cccccc}
\toprule
Method     	& R@1	& R@10  & R@$10^2$  & R@$10^3$  \\ \midrule
from Res4\_3(original) & 58.77 	& 74.18  & 86.20 & 95.33   \\
from Res4\_2   & 65.15 	& 79.21  & 89.01 & 95.84   \\
from Res4\_1   & 70.09    & 82.73   & 90.58  & 96.10 \\
from Res3\_6   & 67.40    & 79.86   & 88.29  & 94.37 \\
from Res3\_5   & 66.46    & 78.85   & 87.43  & 93.84 \\
\bottomrule
\end{tabular}



\caption{Results tail-cut Stanford online products dataset}
\begin{tabular}{cccccc}
\toprule
Method     	& R@1	& R@10  & R@$10^2$  & R@$10^3$  \\ \midrule
from Mixed\_7c(original) & 39.52 	& 54.90  & 70.96 & 87.72   \\
from Mixed\_7b   & 49.87 	& 65.49  & 79.46 & 92.10   \\
from Mixed\_7a   & 54.22    & 69.44   & 81.79  & 92.54 \\
from Mixed\_6e   & 55.53    & 70.62   & 82.86  & 92.92 \\
from Mixed\_6d   & 59.54    & 73.26   & 83.85  & 92.81 \\
from Mixed\_6c   & 61.79    & 75.05   & 84.88  & 92.97 \\

\bottomrule
\end{tabular}
\end{table*}


==> input_tables/sop_cut.tex <==
\begin{table}[]
\centering
\caption{Zero-shot training results of cut-out method on Stanford online products}
% \resizebox{0.5\textwidth}{!}{
\label{table:sop-cut}
\begin{tabular}{lccccc}
\toprule
Method     	& R@1	& R@10  & R@$10^2$  & R@$10^3$  \\ \midrule
Original & 58.77 	& 74.18  & 86.20 & 95.33   \\
Cut 16   & 65.15 	& 79.21  & 89.01 & 95.84   \\
Cut 16~\&~15   & \textbf{70.09} & \textbf{82.73} & \textbf{90.58} & \textbf{96.10} \\
Cut 16~$\sim$14   & 67.40    & 79.86   & 88.29  & 94.37 \\
Cut 16~$\sim$13   & 66.46    & 78.85   & 87.43  & 93.84 \\
\bottomrule
\end{tabular}
% }
\end{table}


==> input_tables/sota_retrieval_sopinshop.tex <==
\begin{table*}[t]
\centering
\caption{Comparison with state-of-the-art methods on image retrieval datasets (Recall@\textit{K} Score)} %(ResNet-50 used, $\dagger$H means head of hydra structure)}
\label{table:sota_retrieval}
\vspace{+1mm}
% \footnotesize{
% \resizebox{1\textwidth}{!}{
\begin{tabular}{ll|cccc|cccc}
\toprule
      & & \multicolumn{4}{c|}{Stanford online products} & \multicolumn{4}{c}{Inshop}\\ 
Method   & Network    & 1     & 10 & $10^{2}$  &$10^{3}$ & 1     & 10  &20  &30 \\ \midrule
%baseline& 89.3 &97.5  & 98.4          & 81.8	& 92.3  & 96.7      \\
A-BIER &Inception-v1       & 74.2 & 86.9  & 94.0 & 97.8 & 83.1 & 95.1 & 96.9 &97.5 \\
DREML &Inception-v3     &-&-&-&-      &78.4&93.7&95.8&96.7                                                 \\
ABE-8 &Inception-v1       & 76.3	& 88.4  & 94.8 &98.2      & 87.3 &96.7  & 97.9& 98.2  \\             
NormSoft &ResNet-50       & 79.5 & 91.5 & 96.7& -  & 89.4 & 97.8 & {98.7}& \textbf{99.0} \\
Margin &ResNet-50   & 72.7 & 86.2 & 93.8&  98.0             &-&-&-&-             \\
MS &Inception-v1        & 78.2 & 90.5 & 96.0& 98.7       & 89.7 & 97.9 & 98.5& 98.8  \\ 
SCHM &Inception-v1       & 77.6 & 89.1 & 94.7& -      & 91.9 & 98.0 & {98.7}&  \textbf{99.0}   \\ 
BFE &ResNet-50         & 83.0 & {93.3} & \textbf{97.3} &\textbf{99.2}    & 89.1 & 96.3 & 97.6 & 98.5   \\ 
Proxy-Anchor &BN-Inception & 79.1 &90.8 & 96.2 & 98.7          & 91.5 & 98.1 & \textbf{98.8} & \textbf{99.0}   \\ \midrule

\textbf{Pruning only}	  &ResNet-50         & 83.3 	& 92.9  & 96.7 & 98.6    & 88.1 & 97.1  & 97.9 & 98.4     \\
\textbf{Proposed} &ResNet-50   	& \textbf{85.0}    & \textbf{93.8}   & 97.1  & 98.9 	& \textbf{92.1}    & \textbf{98.1}  & 98.6 & 98.9   \\ \bottomrule
\end{tabular}
% }
 \vspace{-0.2cm}
\end{table*}



